Efficient Diffusion on Region Manifolds: Recovering Small Objects with Compact CNN Representations

Query expansion is a popular method to improve the quality of image retrieval with both conventional and CNN representations. It has been so far limited to global image similarity. This work focuses on diffusion, a mechanism that captures the image manifold in the feature space. The diffusion is carried out on descriptors of overlapping image regions rather than on a global image descriptor like in previous approaches. An efficient off-line stage allows optional reduction in the number of stored regions. In the on-line stage, the proposed handling of unseen queries in the indexing stage removes additional computation to adjust the precomputed data. We perform diffusion through a sparse linear system solver, yielding practical query times well below one second. Experimentally, we observe a significant boost in performance of image retrieval with compact CNN descriptors on standard benchmarks, especially when the query object covers only a small part of the image. Small objects have been a common failure case of CNN-based retrieval.

==> ext-plots.tex <==
\usepackage{tikzextern}
%\usepackage{pgffor}
\newcommand{\extfig}[2]{\tikzsetnextfilename{figs/extern/#1}{#2}}
\newcommand{\extdata}[1]{}


==> instre_ex.tex <==
\def\1query{923}
 \def\2query{75}
 \def\3query{603}
 \def\4query{995}
 \def\5query{552}
 \def\6query{869}
 \def\7query{928}
 \def\8query{57}
 \def\9query{930}
 \def\aquery{649}
 \def\bquery{626}
 \def\cquery{447}
 \def\dquery{501}

\setlength{\fboxsep}{0pt}%
\setlength{\fboxrule}{1.5pt}%

\newcommand{\posIm }[3]{\fcolorbox{green}{green}{\includegraphics[width=1.3cm,height=1.3cm]{figs/selected/#1_#3_#2.jpg}}}
\newcommand{\negIm }[3]{\fcolorbox{red}{red}{\includegraphics[width=1.3cm,height=1.3cm]{figs/selected/#1_#3_#2.jpg}}}
\newcommand{\qIm }[1]{\includegraphics[width=1.3cm,height=1.3cm]{figs/selected/#1_bbx.jpg}}

\begin{table*}
  \label{tab:instreEx}
\begin{center}
   \begin{tabular}
   {*{11}{@{\sssp}c@{\sssp}}}
   
%%%
%\qIm{\1query}	&\posIm{\1query}{1}{L}	&\posIm{\1query}{2}{L}	&\posIm{\1query}{3}{L}	&\posIm{\1query}{4}{L}	&\posIm{\1query}{5}{L}	&\posIm{\1query}{6}{L}	&\posIm{\1query}{7}{L}	&\posIm{\1query}{8}{L}	&\posIm{\1query}{9}{L}	&\posIm{\1query}{10}{L}  \\

%	&\posIm{\1query}{1}{G}	&\negIm{\1query}{2}{G}	&\posIm{\1query}{3}{G}	&\negIm{\1query}{4}{G}	&\negIm{\1query}{5}{G}	&\negIm{\1query}{6}{G}	&\negIm{\1query}{7}{G}	&\posIm{\1query}{8}{G}	&\posIm{\1query}{9}{G}	&\negIm{\1query}{10}{G} \\ 

%	&\posIm{\1query}{1}{S}	&\negIm{\1query}{2}{S}	&\negIm{\1query}{3}{S}	&\negIm{\1query}{4}{S}	&\negIm{\1query}{5}{S}	&\posIm{\1query}{6}{S}	&\negIm{\1query}{7}{S}	&\negIm{\1query}{8}{S}	&\negIm{\1query}{9}{S}	&\negIm{\1query}{10}{S} \\ 

%%%
%\qIm{\2query}	&\posIm{\2query}{1}{L}	&\posIm{\2query}{2}{L}	&\posIm{\2query}{3}{L}	&\posIm{\2query}{4}{L}	&\posIm{\2query}{5}{L}	&\posIm{\2query}{6}{L}	&\posIm{\2query}{7}{L}	&\posIm{\2query}{8}{L}	&\posIm{\2query}{9}{L}	&\posIm{\2query}{10}{L}  \\
%
%	&\posIm{\2query}{1}{G}	&\negIm{\2query}{2}{G}	&\negIm{\2query}{3}{G}	&\posIm{\2query}{4}{G}	&\posIm{\2query}{5}{G}	&\posIm{\2query}{6}{G}	&\posIm{\2query}{7}{G}	&\posIm{\2query}{8}{G}	&\posIm{\2query}{9}{G}	&\posIm{\2query}{10}{G} \\ 
%
%	&\negIm{\2query}{1}{S}	&\posIm{\2query}{2}{S}	&\negIm{\2query}{3}{S}	&\posIm{\2query}{4}{S}	&\negIm{\2query}{5}{S}	&\negIm{\2query}{6}{S}	&\negIm{\2query}{7}{S}	&\negIm{\2query}{8}{S}	&\negIm{\2query}{9}{S}	&\negIm{\2query}{10}{S} \\ 

%%%
%\qIm{\3query}	&\posIm{\3query}{1}{L}	&\posIm{\3query}{2}{L}	&\posIm{\3query}{3}{L}	&\posIm{\3query}{4}{L}	&\posIm{\3query}{5}{L}	&\posIm{\3query}{6}{L}	&\posIm{\3query}{7}{L}	&\posIm{\3query}{8}{L}	&\posIm{\3query}{9}{L}	&\posIm{\3query}{10}{L}  \\
%
%	&\posIm{\3query}{1}{G}	&\posIm{\3query}{2}{G}	&\posIm{\3query}{3}{G}	&\posIm{\3query}{4}{G}	&\posIm{\3query}{5}{G}	&\negIm{\3query}{6}{G}	&\posIm{\3query}{7}{G}	&\negIm{\3query}{8}{G}	&\posIm{\3query}{9}{G}	&\negIm{\3query}{10}{G} \\ 
%
%	&\posIm{\3query}{1}{S}	&\posIm{\3query}{2}{S}	&\negIm{\3query}{3}{S}	&\posIm{\3query}{4}{S}	&\posIm{\3query}{5}{S}	&\negIm{\3query}{6}{S}	&\posIm{\3query}{7}{S}	&\posIm{\3query}{8}{S}	&\negIm{\3query}{9}{S}	&\negIm{\3query}{10}{S} \\ 

%%%
\qIm{\4query}	&\posIm{\4query}{1}{L}	&\posIm{\4query}{2}{L}	&\posIm{\4query}{3}{L}	&\posIm{\4query}{4}{L}	&\posIm{\4query}{5}{L}	&\posIm{\4query}{6}{L}	&\posIm{\4query}{7}{L}	&\posIm{\4query}{8}{L}	&\posIm{\4query}{9}{L}	&\posIm{\4query}{10}{L} \rotatebox{90}{~~~ours} \\

%	&\posIm{\4query}{1}{G}	&\posIm{\4query}{2}{G}	&\posIm{\4query}{3}{G}	&\negIm{\4query}{4}{G}	&\negIm{\4query}{5}{G}	&\posIm{\4query}{6}{G}	&\posIm{\4query}{7}{G}	&\posIm{\4query}{8}{G}	&\posIm{\4query}{9}{G}	&\posIm{\4query}{10}{G} \\ 

	&\posIm{\4query}{1}{S}	&\posIm{\4query}{2}{S}	&\posIm{\4query}{3}{S}	&\negIm{\4query}{4}{S}	&\negIm{\4query}{5}{S}	&\negIm{\4query}{6}{S}	&\negIm{\4query}{7}{S}	&\posIm{\4query}{8}{S}	&\posIm{\4query}{9}{S}	&\posIm{\4query}{10}{S} \rotatebox{90}{~baseline}\\ 

%%%
%\qIm{\5query}	&\posIm{\5query}{1}{L}	&\posIm{\5query}{2}{L}	&\posIm{\5query}{3}{L}	&\posIm{\5query}{4}{L}	&\posIm{\5query}{5}{L}	&\posIm{\5query}{6}{L}	&\posIm{\5query}{7}{L}	&\posIm{\5query}{8}{L}	&\posIm{\5query}{9}{L}	&\posIm{\5query}{10}{L}  \\
%
%	&\posIm{\5query}{1}{G}	&\posIm{\5query}{2}{G}	&\posIm{\5query}{3}{G}	&\posIm{\5query}{4}{G}	&\negIm{\5query}{5}{G}	&\posIm{\5query}{6}{G}	&\negIm{\5query}{7}{G}	&\posIm{\5query}{8}{G}	&\posIm{\5query}{9}{G}	&\posIm{\5query}{10}{G} \\ 
%
%	&\posIm{\5query}{1}{S}	&\posIm{\5query}{2}{S}	&\posIm{\5query}{3}{S}	&\posIm{\5query}{4}{S}	&\posIm{\5query}{5}{S}	&\negIm{\5query}{6}{S}	&\negIm{\5query}{7}{S}	&\posIm{\5query}{8}{S}	&\posIm{\5query}{9}{S}	&\negIm{\5query}{10}{S} \\ 


\qIm{\6query}	&\posIm{\6query}{1}{L}	&\posIm{\6query}{2}{L}	&\posIm{\6query}{3}{L}	&\posIm{\6query}{4}{L}	&\posIm{\6query}{5}{L}	&\posIm{\6query}{6}{L}	&\posIm{\6query}{7}{L}	&\posIm{\6query}{8}{L}	&\posIm{\6query}{9}{L}	&\posIm{\6query}{10}{L}  \rotatebox{90}{~~~ours}\\

%	&\posIm{\6query}{1}{G}	&\posIm{\6query}{2}{G}	&\posIm{\6query}{3}{G}	&\posIm{\6query}{4}{G}	&\posIm{\6query}{5}{G}	&\posIm{\6query}{6}{G}	&\posIm{\6query}{7}{G}	&\posIm{\6query}{8}{G}	&\negIm{\6query}{9}{G}	&\negIm{\6query}{10}{G} \\ 

	&\posIm{\6query}{1}{S}	&\posIm{\6query}{2}{S}	&\posIm{\6query}{3}{S}	&\posIm{\6query}{4}{S}	&\posIm{\6query}{5}{S}	&\posIm{\6query}{6}{S}	&\negIm{\6query}{7}{S}	&\negIm{\6query}{8}{S}	&\posIm{\6query}{9}{S}	&\negIm{\6query}{10}{S} \rotatebox{90}{~baseline}\\ 

%%%
\qIm{\7query}	&\posIm{\7query}{1}{L}	&\posIm{\7query}{2}{L}	&\posIm{\7query}{3}{L}	&\posIm{\7query}{4}{L}	&\posIm{\7query}{5}{L}	&\posIm{\7query}{6}{L}	&\posIm{\7query}{7}{L}	&\posIm{\7query}{8}{L}	&\posIm{\7query}{9}{L}	&\posIm{\7query}{10}{L}  \rotatebox{90}{~~~ours}\\

%	&\negIm{\7query}{1}{G}	&\posIm{\7query}{2}{G}	&\negIm{\7query}{3}{G}	&\negIm{\7query}{4}{G}	&\negIm{\7query}{5}{G}	&\negIm{\7query}{6}{G}	&\posIm{\7query}{7}{G}	&\posIm{\7query}{8}{G}	&\negIm{\7query}{9}{G}	&\negIm{\7query}{10}{G} \\ 

	&\posIm{\7query}{1}{S}	&\negIm{\7query}{2}{S}	&\negIm{\7query}{3}{S}	&\negIm{\7query}{4}{S}	&\posIm{\7query}{5}{S}	&\negIm{\7query}{6}{S}	&\negIm{\7query}{7}{S}	&\posIm{\7query}{8}{S}	&\negIm{\7query}{9}{S}	&\negIm{\7query}{10}{S} \rotatebox{90}{~baseline}\\ 

  \end{tabular}
    \caption{Retrieval examples on INSTRE dataset. The query image is shown on the left and the query region is drawn in magenta color. Top row shows top retrieved images with our method (regional diffusion), while bottom rows shows top retrieval images with the baseline global descriptor (R-MAC) and nearest neighbor search. Correct (wrong) results are shown in green (red) border.}
\end{center}
\vspace{-10pt}
\end{table*}


%\begin{table*}
%  \label{tab:instreEx}
%\begin{center}
%   \begin{tabular}
%   {*{11}{@{\sssp}c@{\sssp}}}
%
%%%%
%\qIm{\6query}	&\posIm{\6query}{1}{L}	&\posIm{\6query}{2}{L}	&\posIm{\6query}{3}{L}	&\posIm{\6query}{4}{L}	&\posIm{\6query}{5}{L}	&\posIm{\6query}{6}{L}	&\posIm{\6query}{7}{L}	&\posIm{\6query}{8}{L}	&\posIm{\6query}{9}{L}	&\posIm{\6query}{10}{L}  \\
%
%	&\posIm{\6query}{1}{G}	&\posIm{\6query}{2}{G}	&\posIm{\6query}{3}{G}	&\posIm{\6query}{4}{G}	&\posIm{\6query}{5}{G}	&\posIm{\6query}{6}{G}	&\posIm{\6query}{7}{G}	&\posIm{\6query}{8}{G}	&\negIm{\6query}{9}{G}	&\negIm{\6query}{10}{G} \\ 
%
%	&\posIm{\6query}{1}{S}	&\posIm{\6query}{2}{S}	&\posIm{\6query}{3}{S}	&\posIm{\6query}{4}{S}	&\posIm{\6query}{5}{S}	&\posIm{\6query}{6}{S}	&\negIm{\6query}{7}{S}	&\negIm{\6query}{8}{S}	&\posIm{\6query}{9}{S}	&\negIm{\6query}{10}{S} \\ 
%
%%%%
%\qIm{\7query}	&\posIm{\7query}{1}{L}	&\posIm{\7query}{2}{L}	&\posIm{\7query}{3}{L}	&\posIm{\7query}{4}{L}	&\posIm{\7query}{5}{L}	&\posIm{\7query}{6}{L}	&\posIm{\7query}{7}{L}	&\posIm{\7query}{8}{L}	&\posIm{\7query}{9}{L}	&\posIm{\7query}{10}{L}  \\
%
%	&\negIm{\7query}{1}{G}	&\posIm{\7query}{2}{G}	&\negIm{\7query}{3}{G}	&\negIm{\7query}{4}{G}	&\negIm{\7query}{5}{G}	&\negIm{\7query}{6}{G}	&\posIm{\7query}{7}{G}	&\posIm{\7query}{8}{G}	&\negIm{\7query}{9}{G}	&\negIm{\7query}{10}{G} \\ 
%
%	&\posIm{\7query}{1}{S}	&\negIm{\7query}{2}{S}	&\negIm{\7query}{3}{S}	&\negIm{\7query}{4}{S}	&\posIm{\7query}{5}{S}	&\negIm{\7query}{6}{S}	&\negIm{\7query}{7}{S}	&\posIm{\7query}{8}{S}	&\negIm{\7query}{9}{S}	&\negIm{\7query}{10}{S} \\ 
%
%%%%
%\qIm{\8query}	&\posIm{\8query}{1}{L}	&\posIm{\8query}{2}{L}	&\posIm{\8query}{3}{L}	&\posIm{\8query}{4}{L}	&\posIm{\8query}{5}{L}	&\posIm{\8query}{6}{L}	&\posIm{\8query}{7}{L}	&\posIm{\8query}{8}{L}	&\posIm{\8query}{9}{L}	&\posIm{\8query}{10}{L}  \\
%
%	&\posIm{\8query}{1}{G}	&\posIm{\8query}{2}{G}	&\negIm{\8query}{3}{G}	&\negIm{\8query}{4}{G}	&\posIm{\8query}{5}{G}	&\posIm{\8query}{6}{G}	&\negIm{\8query}{7}{G}	&\negIm{\8query}{8}{G}	&\negIm{\8query}{9}{G}	&\negIm{\8query}{10}{G} \\ 
%
%	&\posIm{\8query}{1}{S}	&\posIm{\8query}{2}{S}	&\posIm{\8query}{3}{S}	&\negIm{\8query}{4}{S}	&\posIm{\8query}{5}{S}	&\negIm{\8query}{6}{S}	&\negIm{\8query}{7}{S}	&\negIm{\8query}{8}{S}	&\negIm{\8query}{9}{S}	&\negIm{\8query}{10}{S} \\ 
%
%%%%
%\qIm{\9query}	&\posIm{\9query}{1}{L}	&\posIm{\9query}{2}{L}	&\posIm{\9query}{3}{L}	&\posIm{\9query}{4}{L}	&\posIm{\9query}{5}{L}	&\posIm{\9query}{6}{L}	&\posIm{\9query}{7}{L}	&\posIm{\9query}{8}{L}	&\posIm{\9query}{9}{L}	&\posIm{\9query}{10}{L}  \\
%
%	&\posIm{\9query}{1}{G}	&\posIm{\9query}{2}{G}	&\posIm{\9query}{3}{G}	&\negIm{\9query}{4}{G}	&\posIm{\9query}{5}{G}	&\negIm{\9query}{6}{G}	&\negIm{\9query}{7}{G}	&\negIm{\9query}{8}{G}	&\negIm{\9query}{9}{G}	&\negIm{\9query}{10}{G} \\ 
%
%	&\posIm{\9query}{1}{S}	&\posIm{\9query}{2}{S}	&\posIm{\9query}{3}{S}	&\posIm{\9query}{4}{S}	&\negIm{\9query}{5}{S}	&\negIm{\9query}{6}{S}	&\negIm{\9query}{7}{S}	&\negIm{\9query}{8}{S}	&\negIm{\9query}{9}{S}	&\negIm{\9query}{10}{S} \\ 
%
%
%
%  \end{tabular}
%    \caption{Instre examples Part 2.}
%\end{center}
%\vspace{-10pt}
%\end{table*}
%
%
%\begin{table*}
%  \label{tab:instreEx}
%\begin{center}
%   \begin{tabular}
%   {*{11}{@{\sssp}c@{\sssp}}}
%
%%%%
%\qIm{\aquery}	&\posIm{\aquery}{1}{L}	&\posIm{\aquery}{2}{L}	&\posIm{\aquery}{3}{L}	&\posIm{\aquery}{4}{L}	&\posIm{\aquery}{5}{L}	&\posIm{\aquery}{6}{L}	&\posIm{\aquery}{7}{L}	&\posIm{\aquery}{8}{L}	&\posIm{\aquery}{9}{L}	&\posIm{\aquery}{10}{L}  \\
%
%	&\posIm{\aquery}{1}{G}	&\posIm{\aquery}{2}{G}	&\negIm{\aquery}{3}{G}	&\posIm{\aquery}{4}{G}	&\posIm{\aquery}{5}{G}	&\posIm{\aquery}{6}{G}	&\negIm{\aquery}{7}{G}	&\negIm{\aquery}{8}{G}	&\negIm{\aquery}{9}{G}	&\negIm{\aquery}{10}{G} \\ 
%
%	&\posIm{\aquery}{1}{S}	&\posIm{\aquery}{2}{S}	&\posIm{\aquery}{3}{S}	&\posIm{\aquery}{4}{S}	&\negIm{\aquery}{5}{S}	&\posIm{\aquery}{6}{S}	&\negIm{\aquery}{7}{S}	&\negIm{\aquery}{8}{S}	&\negIm{\aquery}{9}{S}	&\negIm{\aquery}{10}{S} \\ 
%
%%%%
%\qIm{\bquery}	&\posIm{\bquery}{1}{L}	&\posIm{\bquery}{2}{L}	&\posIm{\bquery}{3}{L}	&\posIm{\bquery}{4}{L}	&\posIm{\bquery}{5}{L}	&\posIm{\bquery}{6}{L}	&\posIm{\bquery}{7}{L}	&\posIm{\bquery}{8}{L}	&\posIm{\bquery}{9}{L}	&\posIm{\bquery}{10}{L}  \\
%
%	&\posIm{\bquery}{1}{G}	&\posIm{\bquery}{2}{G}	&\posIm{\bquery}{3}{G}	&\posIm{\bquery}{4}{G}	&\posIm{\bquery}{5}{G}	&\negIm{\bquery}{6}{G}	&\posIm{\bquery}{7}{G}	&\negIm{\bquery}{8}{G}	&\negIm{\bquery}{9}{G}	&\negIm{\bquery}{10}{G} \\ 
%
%	&\posIm{\bquery}{1}{S}	&\posIm{\bquery}{2}{S}	&\posIm{\bquery}{3}{S}	&\posIm{\bquery}{4}{S}	&\posIm{\bquery}{5}{S}	&\negIm{\bquery}{6}{S}	&\negIm{\bquery}{7}{S}	&\posIm{\bquery}{8}{S}	&\negIm{\bquery}{9}{S}	&\negIm{\bquery}{10}{S} \\ 
%
%%%%
%\qIm{\cquery}	&\posIm{\cquery}{1}{L}	&\posIm{\cquery}{2}{L}	&\posIm{\cquery}{3}{L}	&\posIm{\cquery}{4}{L}	&\posIm{\cquery}{5}{L}	&\posIm{\cquery}{6}{L}	&\posIm{\cquery}{7}{L}	&\posIm{\cquery}{8}{L}	&\posIm{\cquery}{9}{L}	&\posIm{\cquery}{10}{L}  \\
%
%	&\posIm{\cquery}{1}{G}	&\posIm{\cquery}{2}{G}	&\posIm{\cquery}{3}{G}	&\posIm{\cquery}{4}{G}	&\posIm{\cquery}{5}{G}	&\posIm{\cquery}{6}{G}	&\negIm{\cquery}{7}{G}	&\posIm{\cquery}{8}{G}	&\negIm{\cquery}{9}{G}	&\negIm{\cquery}{10}{G} \\ 
%
%	&\posIm{\cquery}{1}{S}	&\posIm{\cquery}{2}{S}	&\posIm{\cquery}{3}{S}	&\posIm{\cquery}{4}{S}	&\posIm{\cquery}{5}{S}	&\posIm{\cquery}{6}{S}	&\negIm{\cquery}{7}{S}	&\negIm{\cquery}{8}{S}	&\posIm{\cquery}{9}{S}	&\negIm{\cquery}{10}{S} \\ 
%
%%%%
%\qIm{\dquery}	&\posIm{\dquery}{1}{L}	&\posIm{\dquery}{2}{L}	&\posIm{\dquery}{3}{L}	&\negIm{\dquery}{4}{L}	&\posIm{\dquery}{5}{L}	&\posIm{\dquery}{6}{L}	&\posIm{\dquery}{7}{L}	&\posIm{\dquery}{8}{L}	&\posIm{\dquery}{9}{L}	&\posIm{\dquery}{10}{L}  \\
%
%	&\posIm{\dquery}{1}{G}	&\posIm{\dquery}{2}{G}	&\posIm{\dquery}{3}{G}	&\posIm{\dquery}{4}{G}	&\negIm{\dquery}{5}{G}	&\posIm{\dquery}{6}{G}	&\negIm{\dquery}{7}{G}	&\negIm{\dquery}{8}{G}	&\posIm{\dquery}{9}{G}	&\negIm{\dquery}{10}{G} \\ 
%
%	&\posIm{\dquery}{1}{S}	&\posIm{\dquery}{2}{S}	&\posIm{\dquery}{3}{S}	&\negIm{\dquery}{4}{S}	&\posIm{\dquery}{5}{S}	&\posIm{\dquery}{6}{S}	&\posIm{\dquery}{7}{S}	&\negIm{\dquery}{8}{S}	&\negIm{\dquery}{9}{S}	&\negIm{\dquery}{10}{S} \\ 
%
%  \end{tabular}
%    \caption{Instre examples Part 3.}
%\end{center}
%\vspace{-10pt}
%\end{table*}


==> instre_fail_ex.tex <==
\def\1query{1213}

\newcommand{\posFailIm }[3]{\fcolorbox{green}{green}{\makebox(35,35){\includegraphics[width=1.3cm,height=1.3cm]{figs/selected/fail_#1_#3_#2.jpg}}}}
\newcommand{\negFailIm }[3]{\fcolorbox{red}{red}{\makebox(35,35){\includegraphics[width=1.3cm,height=1.3cm]{figs/selected/fail_#1_#3_#2.jpg}}}}
\newcommand{\qFailIm }[1]{\fcolorbox{magenta}{magenta}{\makebox(35,35){\includegraphics[width=1.3cm,height=1.3cm]{figs/selected/fail_#1_bbx.jpg}}}}

\begin{table*}
  \label{tab:instreFailEx}
\begin{center}
   \begin{tabular}
   {*{11}{@{\sssp}c@{\sssp}}}
   
%%%
\qFailIm{\1query}	&\posFailIm{\1query}{1}{L}	&\negFailIm{\1query}{2}{L}	&\posFailIm{\1query}{3}{L}	&\posFailIm{\1query}{4}{L}	&\posFailIm{\1query}{5}{L}	&\negFailIm{\1query}{6}{L}	&\negFailIm{\1query}{7}{L}	&\negFailIm{\1query}{8}{L}	&\negFailIm{\1query}{9}{L}	&\negFailIm{\1query}{10}{L}  \\

%	&\posFailIm{\1query}{1}{G}	&\posFailIm{\1query}{2}{G}	&\posFailIm{\1query}{3}{G}	&\posFailIm{\1query}{4}{G}	&\posFailIm{\1query}{5}{G}	&\posFailIm{\1query}{6}{G}	&\posFailIm{\1query}{7}{G}	&\posFailIm{\1query}{8}{G}	&\posFailIm{\1query}{9}{G}	&\posFailIm{\1query}{10}{G} \\ 

	&\posFailIm{\1query}{1}{S}	&\posFailIm{\1query}{2}{S}	&\posFailIm{\1query}{3}{S}	&\posFailIm{\1query}{4}{S}	&\posFailIm{\1query}{5}{S}	&\posFailIm{\1query}{6}{S}	&\posFailIm{\1query}{7}{S}	&\posFailIm{\1query}{8}{S}	&\posFailIm{\1query}{9}{S}	&\posFailIm{\1query}{10}{S} \\ 

  \end{tabular}
    \caption{An example where regional diffusion fails in INSTRE dataset. Bounding box contains a keychain object, and regional diffusion retrieves other objects that contain chain. }
\end{center}
\vspace{-10pt}
\end{table*}


==> instre_intro.tex <==
\def\1query{923}

\setlength{\fboxsep}{0pt}%
\setlength{\fboxrule}{1.5pt}%

\newcommand{\posIntroIm }[3]{\fcolorbox{green}{green}{\includegraphics[width=0.8cm,height=0.8cm]{figs/selected/#1_#3_#2.jpg}}}
\newcommand{\negIntroIm }[3]{\fcolorbox{red}{red}{\includegraphics[width=0.8cm,height=0.8cm]{figs/selected/#1_#3_#2.jpg}}}
\newcommand{\qIntroIm }[1]{\includegraphics[width=1.3cm,height=1.3cm]{figs/selected/#1_bbx.jpg}}



\begin{figure}
  \label{fig:instreIntro}
\begin{center}
   \begin{tabular}
   { @{\sssp}c@{\sssp}  c@{\sssp}  @{\sssp}c@{\sssp} @{\sssp}c c@{\sssp} @{\sssp}c@{\sssp} @{\sssp}c@{\sssp}}

%%%
%\qIntroIm{\1query}	&\posIntroIm{\1query}{1}{L}	&\posIntroIm{\1query}{2}{L}	&\posIntroIm{\1query}{3}{L}	&\posIntroIm{\1query}{4}{L}	&\posIntroIm{\1query}{5}{L}	&\posIntroIm{\1query}{6}{L}	&\posIntroIm{\1query}{7}{L}	&\posIntroIm{\1query}{8}{L}	&\posIntroIm{\1query}{9}{L}	&\posIntroIm{\1query}{10}{L}  \\
%
%	&\posIntroIm{\1query}{1}{S}	&\negIntroIm{\1query}{2}{S}	&\negIntroIm{\1query}{3}{S}	&\negIntroIm{\1query}{4}{S}	&\negIntroIm{\1query}{5}{S}	&\posIntroIm{\1query}{6}{S}	&\negIntroIm{\1query}{7}{S}	&\negIntroIm{\1query}{8}{S}	&\negIntroIm{\1query}{9}{S}	&\negIntroIm{\1query}{10}{S} \\


\multirow{ 5}{*}{\qIntroIm{\1query}	}~~~ & \posIntroIm{\1query}{1}{S}  & \negIntroIm{\1query}{2}{S}  & \negIntroIm{\1query}{3}{S} &\posIntroIm{\1query}{1}{L}	&\posIntroIm{\1query}{2}{L}	&\posIntroIm{\1query}{3}{L} \\

		&  \negIntroIm{\1query}{4}{S}	&\negIntroIm{\1query}{5}{S}	&\posIntroIm{\1query}{6}{S}	&  \posIntroIm{\1query}{4}{L}	&\posIntroIm{\1query}{5}{L}	&\posIntroIm{\1query}{6}{L}	\\

		&	\negIntroIm{\1query}{7}{S}	&\negIntroIm{\1query}{8}{S}	&\negIntroIm{\1query}{9}{S}  & \posIntroIm{\1query}{7}{L}	&\posIntroIm{\1query}{8}{L}	&\posIntroIm{\1query}{9}{L} \\


  \end{tabular}
    \caption{\textit{Left:} Query region defined by bounding box. \textit{Middle:} Top retrieved images using global image representation and nearest neighbor search. \textit{Right:} Top retrieved images with the proposed regional diffusion.}
\end{center}
\vspace{-10pt}
\end{figure}




==> no-plots.tex <==
\newcommand{\extfig}[2]{!}
\newcommand{\extdata}[1]{}

